Learning to Reconstruct 3D Manhattan Wireframes from a Single Image

In this paper, we propose a method to obtain a compact and accurate 3D wireframe representation from a single image by effectively exploiting global structural regularities. Our method trains a convolutional neural network to simultaneously detect salient junctions and straight lines, as well as predict their 3D depth and vanishing points. Compared with the state-of-the-art learning-based wireframe detection methods, our network is simpler and more unified, leading to better 2D wireframe detection. With global structural priors from parallelism, our method further reconstructs a full 3D wireframe model, a compact vector representation suitable for a variety of high-level vision tasks such as AR and CAD. We conduct extensive evaluations on a large synthetic dataset of urban scenes as well as real images. Our code and datasets have been made public at https://github.com/zhou13/shapeunity.

==> conclusion.tex <==
\section{Future Work}
\label{sec:conclusion}


We have shown the feasibility of learning and detecting high-level geometric features such as a wireframe of lines and junctions for the recovery of compact 3D geometry of an urban scene, even from a single view. To further improve the performance of our system and apply to diverse real-world scenes (both indoors and outdoors), we need new datasets with high-quality images and high-level 3D models of such scenes. We also plan to extend our wireframe representations to accommodate curves, surfaces, and more complex geometric primitives, and generalize the 3D reconstruction methods to handle scenes that are not entirely Manhattan. %



==> cvpr.tex <==
\def\cvprPaperID{2132}
\def\httilde{\mbox{\tt\raisebox{-.5ex}{\symbol{126}}}}
\ifcvprfinal\pagestyle{empty}\fi


==> interface.tex <==
\section{User Interface}
\label{sec:interface}

\note{
People like to know what you have done before how it is done.

For HCI papers it is common to start with the user interface or usage scenarios.
Even for a very theoretical paper, we can summarize the main equations/methods/applications/implications here, before diving into technical details.
}%

On top of automatic system results which might not be completely correct, users can correct the lines and contours.
They can also edit the shapes.

\liyi{(June 8, 2018)
Do we want to handle only individual images or also consider multiple frames/videos?
}%


==> intern.tex <==
\section{Internship}

\subsection{Intro talk}

INTERN SPEAKER: Yichao Zhou
 
MENTORS/COLLABORATORS: Qi Sun, Zhili Chen, and Li-Yi Wei
 
TITLE:  Wireframe3D --- Data-driven Global 3D Reconstruction from Photos
 
ABSTRACT:  
Man-made environments (both indoor and outdoor) are rich of large-scale structural regularities such as straight lines, parallelism, orthogonality, symmetry, and smooth curves and surfaces. However, conventional 3D reconstruction methods (such as structure from motion) utilize only local features (such as corner-like features) and cannot benefit from such strong global structural priors. In this project, we aim to exploit such large-scale structural regularities for recovering accurate large-scale 3D geometry of a scene and objects in it. Instead of generating point clouds or meshes, we are interested in obtaining a high-level vectorized representation of the geometry, in terms of lines, planes, curves or surfaces. Such representations would be largely suitable for purposes such as virtual reality and augmented reality.
 
BIO:
Yichao Zhou is a Ph.D student at Center of Augmented Cognition and Visual Computing Lab in University of California, Berkeley.  His research interests lie in 3D vision, computer graphics, and parallel computing.



==> limitation_fig.tex <==
\begin{figure}[tbh!p]
  \centering
  \warning{TODO}
  \caption[Limitation case.]
  {%
Our method cannot reconstruct curved wireframes or objects lacking definitive contours.
\liyi{(November 14, 2018)
There is an important distinction we should clarify: reconstruct only Manhattan parts of an image of a general scene, or complete failure if the input image is not sufficiently Manhattan.
My understanding is that our method is the former case, and thus I have written the paper title accordingly.
}%
\yichao{if it is too non-manhattan, it is likely the algorithm will fail due to the error in vanish point detection.}
  }
\label{fig:limitation}
\end{figure}


==> network_fig.tex <==
\begin{figure}[thb]
    \centering
    \includegraphics[draft,width=0.99\linewidth]{figs/network.pdf}
    \caption{Our network structure.}
    \label{fig:network}
\end{figure}


==> prior.tex <==
\section{Related Work}
\label{sec:prior}

\liyi{(October 2, 2018)
Put \cite{Zou:2018:LNR} and related works (like RoomNet) somewhere.
}%


\paragraph{High level reconstruction}

Capturing detailed geometry is a challenging problem and often unnecessary for many applications.
A variety of methods have been proposed to capture high level coarse structures in 2D \cite{Huang:2018:LPW} and 3D \cite{Huang:2017:TCS}.
Our method follow this line to reconstruct Manhattan worlds in 3D.

\note{TODO: Add structure from motion literature.}

Current off-the-shelf commercial solutions for indoor physical scene reconstruction, such as the Microsoft Mixed Realty Toolkit for AR scenarios\footnote{https://github.com/Microsoft/MixedRealityToolkit-Unity}, can reach high quality and performance.  However, those systems usually require depth camera which currently is not common among mobile devices or rely on specific object query.  In addition, their methods are not suitable for outdoor scenes reconstruction due to the limitation of depth sensors.

\cite{Kelly:2017:BLS} reconstructs noiseless and high quality large scale urban scenes. However, the system requires GIS footprint and 3D mesh as input, thus becomes impractical for common AR applications in indoor scenes with non-architectural elements.

\cite{Liu:2017:IRW} reconstructs the structure of some speical items such as wired artworks.

With the recent progress made in the deep learning community, there are a lot of researches forced on data-driven method.  Those methods typically required training on a pre-exist database.  \cite{Liu:2018:Planenet} \cite{Groueix:2018:AN} \note{TODO: Add more paper for single-image depth recovery.}

Our method extend the work of \cite{Huang:2018:LPW}, which extracted the 2D wireframes for indoor images.  Our 3D wireframe-based reconstruction is similar to the line-based reconstruction methods in SLAM community, which were explored by \cite{Hofer:2017:Efficient,Fleet:2014:Lsd}.

\paragraph{Shape fitting to curves}

\cite{Zheng:2012:IIC,Xu:2014:TCN,Pan:2015:FAS,Li:2017:BMF,Han:2017:DDL,Su:2018:ISN}

\liyi{(June 14, 2018)
This is related to our 2D-to-3D lifting part in terms of novelty and methodology.
}%

\paragraph{Learning-based methods}
\cite{Eslami:2018:NSR} learn a sparse scene representation from multiple rendered views.
\note{(June 15, 2018)
\cite{Eslami:2018:NSR:blog} is the corresponding blog post.
}

\paragraph{Appearance capture}

\cite{Bi:2017:POI}

\yichao{
\cite{Bi:2017:POI}  XXX: I think this paper is for generate texture for a existing mesh, rather than doing the 3D reconstruction, right?
}%

\paragraph{Wireframe representation} \cite{Huang:2018:LPW}

\hqi{
Here we should carefully evaluate the difference compared width \cite{Huang:2018:LPW}, talk about or contribution.
}

